HealthE: Classifying Entities in Online Textual Health Advice

The processing of entities in natural language is essential to many medical NLP systems. Unfortunately, existing datasets vastly under-represent the entities required to model public health relevant texts such as health advice often found on sites like WebMD. People rely on such information for personal health management and clinically relevant decision making. In this work, we release a new annotated dataset, HealthE, consisting of 6,756 health advice. HealthE has a more granular label space compared to existing medical NER corpora and contains annotation for diverse health phrases. Additionally, we introduce a new health entity classification model, EP S-BERT, which leverages textual context patterns in the classification of entity classes. EP S-BERT provides a 4-point increase in F1 score over the nearest baseline and a 34-point increase in F1 when compared to off-the-shelf medical NER tools trained to extract disease and medication mentions from clinical texts. All code and data are publicly available on Github.

==> Sections/0abstract.tex <==
\begin{abstract}
Importance of area. Description of problem. We introduce HealthE, a new benchmark dataset for approaching this low-resource problem as either a medical entity set expansion (ESE), medical named entity recognition (NER), or medical entity classification (EC) task. We introduce a simple transfer learning approach for medical EC, entity/pattern sentence BERT (EP S-BERT), which utilizes sentence BERT embeddings of entities and contextual patterns for capturing medical entity semantics. We perform comprehensive experiments to show that EP S-BERT outperforms state of the art baseline models in both the EC and pretrained medical NER tasks. Through extensive error analysis of EP S-BERT we discover two core challenges for future work utilizing HealthE.
\end{abstract}

==> Sections/2related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\subsection{Entity Set Expansion}

\begin{itemize}
    \item Explain ESE (lexicon induction)
    \item Brief bootstrapnet intro (explain that it is SOTA)
\end{itemize}

\subsection{Medical Named Entity Recognition}

\begin{itemize}
    \item Explain previous efforts in MedNER
\end{itemize}

==> Sections/5results.tex <==


\subsection{Error Analysis}
\begin{itemize}
    \item Which classes does the model fail on?
    \item Which classes are commonly confused with each other?
    \item Error labeling - we manually categorize each entity that EP S-BERT misclassified into one of four categories, we have a table for this
\end{itemize}


